On the Presence of Green and Sustainable Software Engineering in Higher Education Curricula

Nowadays, software is pervasive in our everyday lives. Its sustainability and environmental impact have become major factors to be considered in the development of software systems. Millennials-the newer generation of university students-are particularly keen to learn about and contribute to a more sustainable and green society. The need for training on green and sustainable topics in software engineering has been reflected in a number of recent studies. The goal of this paper is to get a first understanding of what is the current state of teaching sustainability in the software engineering community, what are the motivations behind the current state of teaching, and what can be done to improve it. To this end, we report the findings from a targeted survey of 33 academics on the presence of green and sustainable software engineering in higher education. The major findings from the collected data suggest that sustainability is under-represented in the curricula, while the current focus of teaching is on energy efficiency delivered through a fact-based approach. The reasons vary from lack of awareness, teaching material and suitable technologies, to the high effort required to teach sustainability. Finally, we provide recommendations for educators willing to teach sustainability in software engineering that can help to suit millennial students needs.

==> tableI.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\caption{Survey questionnaire}
\begin{tabular}{llccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Section}}                                                                               & \multicolumn{1}{c}{\multirow{2}{*}{Survey Questions}}                                                                                                                                                                                                                                                               & \multicolumn{3}{c}{Type of Answers}                                                                      \\ \cline{3-5} 
\multicolumn{1}{c}{}                                                                                                       & \multicolumn{1}{c}{}                                                                                                                                                                                                                                                                                                & \multicolumn{1}{l}{Single from list} & \multicolumn{1}{l}{Likert scale} & \multicolumn{1}{l}{Other text} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}1. Background \\ information\end{tabular}}                                      & SQ1. What is your nationality?                                                                                                                                                                                                                                                                                      & X                                    &                                  &                                \\ \cline{2-5} 
                                                                                                                           & SQ2. What is your age range?                                                                                                                                                                                                                                                                                        &                                      & X                                &                                \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ3. What is your current\\ position?\end{tabular}                                                                                                                                                                                                                                       & X                                    &                                  &                                \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}2. Green and Sustainable \\ Software Engineering\end{tabular}}                  & \begin{tabular}[c]{@{}l@{}}SQ4. Do you regularly participate in academic events related\\  to software sustainability? If so, which ones?\end{tabular}                                                                                                                                                              &                                      & X                                &                                \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ5. How would you rank the following dimensions: \\ Economic, Environmental, Social, and Technical\end{tabular}                                                                                                                                                                         &                                      & X                                &                                \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ6. How important is the topic of\\ Green and Sustainable Software in the Software Engineering curricula of your university?\end{tabular}                                                                                                                                               & X                                    &                                  & X                              \\ \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}3. Education in \\ Green and Sustainable \\ Software Engineering\end{tabular}} & \begin{tabular}[c]{@{}l@{}}SQ7. Do you currently (or\\ ever) teach any course related to software sustainability?\end{tabular}                                                                                                                                                                                      & X                                    &                                  &                                \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ8. As you do not teach\\ any course focused on sustainable software, do you teach sustainability topics\\ in your traditional software engineering courses?\\  (e.g. in a programming course, best practices for energy-efficient code). \\ If you replied "no", why not?\end{tabular} & X                                    &                                  & X                              \\ \cline{2-5} 
                                                                                                                           & SQ9. What is the name of the course?                                                                                                                                                                                                                                                                                &                                      &                                  & X                              \\ \cline{2-5} 
                                                                                                                           & SQ10. How many students do you have on average?                                                                                                                                                                                                                                                                     &                                      & X                                &                                \\ \cline{2-5} 
                                                                                                                           & SQ11. What is the duration of the course?                                                                                                                                                                                                                                                                           & X                                    &                                  &                                \\ \cline{2-5} 
                                                                                                                           & SQ12. Is the course exam-based or assignment-based?                                                                                                                                                                                                                                                                 & X                                    &                                  &                                \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ13. Do you involve third parties in your course? \\ (e.g. public/private stakeholders).\\ If so, please describe what type of stakeholders and their involvement.\end{tabular}                                                                                                         & X                                    &                                  & X                              \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ14. Compared with other traditional courses\\  how difficult was to design the course(s) on Green and Sustainable Software topics?\\ Please motivate your answer.\end{tabular}                                                                                                         &                                      & X                                & X                              \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ15. Have you faced any\\ problems in designing the course(s) on Green and Sustainable Software topics?\\ If so, which ones?\end{tabular}                                                                                                                                               & X                                    &                                  & X                              \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ16. Which green and sustainable software aspect (s) were the focus of your course(s)?\\ (e.g., Energy, Efficiency,  Maintainability, Social Sustainability, etc)\end{tabular}                                                                                                          &                                      &                                  & X                              \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}4. Ideas and challenges\\ for the future\end{tabular}}                          & SQ17. Do you think there is a need for more courses related to software sustainability                                                                                                                                                                                                                              & X                                    & \multicolumn{1}{l}{}             &                                \\ \cline{2-5} 
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}SQ18. What type of software\\ sustainability courses would you propose in a Software Engineering curricula?\end{tabular}                                                                                                                                                                 & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}             & X                              \\ \cline{2-5} 
                                                                                                                           & SQ19. What challenges, if any, do you see in teaching software sustainability in higher education?                                                                                                                                                                                                                  & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}             & X                              \\ \hline
\end{tabular}
\label{tbl:survey}
\end{table*}

==> tableII.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Summary of results}
\begin{tabular}{llll}
\hline
\multicolumn{2}{l}{Question}                  & \multicolumn{2}{l}{Results} \\ \hline
\#                     & Possible answers     & Answers     & Percentage    \\ \hline
\multirow{13}{*}{SQ1}  & Spain                & 5           & 15.2          \\
                       & Germany              & 5           & 15.2          \\
                       & Portugal             & 4           & 12.1          \\
                       & Italy                & 3           & 9.1           \\
                       & France               & 3           & 9.1           \\
                       & China                & 3           & 9.1           \\
                       & UK                   & 2           & 6.1           \\
                       & Brazil               & 2           & 6.1           \\
                       & United States        & 2           & 6.1           \\
                       & India                & 1           & 3             \\
                       & Colombia             & 1           & 3             \\
                       & Canada               & 1           & 3             \\
                       & Belgio               & 1           & 3             \\ \hline
\multirow{3}{*}{SQ2}   & less than 30         & 8           & 24.2          \\
                       & 30-45                & 17          & 51.5          \\
                       & 45+                  & 8           & 24.2          \\ \hline
\multirow{6}{*}{SQ3}   & Ph.D. student        & 9           & 27.3          \\
                       & Post-doc             & 3           & 9.1           \\
                       & Assistant professor  & 9           & 27.3          \\
                       & Associate professor  & 5           & 15.2          \\
                       & Full professor       & 5           & 15.2          \\
                       & Other                & 2           & 6.1           \\ \hline
\multirow{2}{*}{SQ4}   & Yes                  & 21          & 63.6          \\
                       & No                   & 12          & 36.4          \\ \hline
\multirow{3}{*}{SQ6}   & Very important       & 3           & 9.1           \\
                       & Partially important  & 10          & 30.3          \\
                       & Not important        & 20          & 60.3          \\ \hline
\multirow{2}{*}{SQ7}   & Yes                  & 12          & 36.4          \\
                       & No                   & 21          & 63.6          \\ \hline
\multirow{2}{*}{SQ8}   & Yes                  & 17          & 81            \\
                       & No                   & 4           & 19            \\ \hline
\multirow{4}{*}{SQ10}  & Less than 20         & 8           & 50            \\
                       & Between 20 and 50    & 6           & 37.5          \\
                       & Between 50 and 100   & 1           & 6.3           \\
                       & More than 100        & 1           & 6.3           \\ \hline
\multirow{4}{*}{SQ11}  & Less then a semester & 3           & 18.8          \\
                       & One semesters        & 12          & 75            \\
                       & Two semesters        & 1           & 6.3           \\
                       & Others               & 0           & 0             \\ \hline
\multirow{3}{*}{SQ 12} & Exam-based           & 7           & 43.8          \\
                       & Assignment-based     & 2           & 12.5          \\
                       & Other                & 7           & 43.8          \\ \hline
\multirow{2}{*}{SQ13}  & Yes                  & 3           & 18.8          \\
                       & No                   & 13          & 81.3          \\ \hline
\multirow{4}{*}{SQ14}  & Very difficult       & 4           & 25            \\
                       & Moderately difficult & 9           & 56.3          \\
                       & Slightly difficult   & 1           & 6.3           \\
                       & Not difficult        & 2           & 12.5          \\ \hline
\multirow{2}{*}{SQ15}  & Yes                  & 2           & 12.5          \\
                       & No                   & 14          & 87.5          \\ \hline
\multirow{2}{*}{SQ17}  & Yes                  & 32          & 97            \\
                       & No                   & 1           & 3             \\ \hline
\end{tabular}
\label{tbl:results}
\end{table}
